Unsupervised Behavior Extraction via Random Intent Priors

Reward-free data is abundant and contains rich prior knowledge of human behaviors, but it is not well exploited by offline reinforcement learning (RL) algorithms. In this paper, we propose UBER, an unsupervised approach to extract useful behaviors from offline reward-free datasets via diversified rewards. UBER assigns different pseudo-rewards sampled from a given prior distribution to different agents to extract a diverse set of behaviors, and reuse them as candidate policies to facilitate the learning of new tasks. Perhaps surprisingly, we show that rewards generated from random neural networks are sufficient to extract diverse and useful behaviors, some even close to expert ones. We provide both empirical and theoretical evidence to justify the use of random priors for the reward function. Experiments on multiple benchmarks showcase UBER's ability to learn effective and diverse behavior sets that enhance sample efficiency for online RL, outperforming existing baselines. By reducing reliance on human supervision, UBER broadens the applicability of RL to real-world scenarios with abundant reward-free data.

==> theory_gamma.tex <==
\section{Theoretical Analysis}
This section characterizes the effects of a lower guidance discount factor in offline RL. We first show that a similar regularization effect exists in offline algorithms as in online algorithms. We quantify this effect by providing a performance bound to analyze how other factors like the data size and the coverage coefficient affect this regularization effect. We then show an equivalence between a lower discount factor and the model-based pessimism. This equivalence leads to a performance guarantee with a lower guidance discount factor without other conservative regularizations. These two effects indicate that the discount factor plays a vital role in offline reinforcement learning.

\subsection{Regularization Effect}
As~\citet{jiang2015dependence} suggests, the discount factor acts as a regularization coefficient to bound the complexity of the potential optimal policy class. However, it is unclear what affects the effectiveness of $\gamma$ regularization in the offline setting, especially when the data coverage is poor and the algorithms have additional pessimism. Empirically, we found that the quality and size of the dataset are the main factors that affect the regularization from $\gamma$. To shed light on this observation, we first derive a performance bound in the linear MDP setting for model-free pessimistic algorithms like Algorithm~\ref{alg:1}. The analysis is analogous to~\citep{jin2021pessimism}, but we focus on the discount setting.
% Specifically, we have the following lemma.

\begin{lemma}
    \label{lemma:2}
    Suppose there exists an absolute constant 
    \begin{align}
        \label{eq:event_opt_explore}
        c^\dagger = &\sup_{x\in \RR^d} \frac{x^{\top}\Sigma_{\pi^*,s}x}{x^{\top}\Sigma_{\cD} x} < \infty,
    \end{align}
    for all $s\in\cS$ with probability $1-\xi/2$, where 
    \$&\Sigma_{\cD}~~~=\frac{1}{N}\sum_{\tau=1}^N{\left[\phi(s_\tau,a_\tau)\phi(s_\tau,a_\tau)^\top\right]},\notag\\
     &\Sigma_{\pi^*,s}=\EE_{{\pi^*}}\bigl[\phi(s_t,a_t)\phi(s_t,a_t)^\top\biggiven s_0=s\bigr].
     \$
    % $c^\dagger >0$ such that with probability $1-\xi/2$,
    % \begin{align}
    %     \label{eq:event_opt_explore}
    %     &\frac{1}{N} \cdot\sum_{\tau=1}^N{\phi(s_\tau,a_\tau)\phi(s_\tau,a_\tau)^\top}\succeq  \nonumber \\
    %     &c^\dagger \cdot  \EE_{\pi^*}\bigl[\phi(s_t,a_t)\phi(s_t,a_t)^\top\biggiven s_0=s\bigr], 
    % \end{align}
    % for all $s\in \cS$.

    In Algorithm \ref{alg:1}, we follow Equation~\eqref{eq:empirical_bellman} and~\eqref{eq:linear_uncertainty_quantifier}, and set 
    \begin{equation*}
        \lambda =1,~ \beta= c \cdot d r_{\text{\rm max}}\sqrt{\zeta}/(1-\gamma), ~ \zeta = \log{(4dN/(1-\gamma)\xi)},
    \end{equation*}
    where $c>0$ is an absolute constant  and $\xi \in (0,1)$ is the confidence parameter. Then with probability $1-\xi$, the policy $\widehat{\pi}$ generated by Algorithm~\ref{alg:1} satisfies
    \begin{align*}\label{eq:event_opt_explore_d}
     \text{\rm SubOpt}\big(\widehat{\pi},s;\gamma \big) 
    \leq  \frac{2c r_{\text{\rm max}}}{(1-\gamma)^2} \sqrt{c^\dagger d^3\zeta /N}, \ \forall s\in \cS.
    \end{align*}
    % for all $s\in \cS$.
\end{lemma}
\begin{proof}
    See Appendix~\ref{proof_lemma_1} for a detailed proof.
\end{proof}

Equation~\eqref{eq:event_opt_explore} defines a finite coverage coefficient, namely $c^\dagger$, which represents the maximum ratio between the density of empirical state-action distribution and the density induced from the optimal policy. Intuitively, it represents the quality of the dataset. For example, the \verb|expert| dataset has a low coverage ratio while the \verb|random| dataset may have a high ratio. The probability $1-\xi/2$ for a finite coverage coefficient is measured concerning the data collection process. That is, we are only making assumptions about the data collection process rather than the specific dataset.
The dependence on $\gamma$ in Lemma~\ref{lemma:2} suggests that the performance bound $\text{SubOpt}\big(\widehat{\pi},s;\gamma \big)$ decreases as the discount factor gets lower. However, a lower discount factor also biases the optimal policy, as characterized by the following lemma.

% Based on the theoretical observation, one may choose a very low $\gamma$ to obtain a better performance bound.

\begin{lemma}[\citet{jiang2015dependence}]
    \label{lemma:1}
     For any MDP $M$ with rewards in $[0,r_{\text{\rm max}}]$, $\forall \pi: \mathcal{S}\times\mathcal{A}\rightarrow \mathbb{R}$ and $\gamma\leq \gamma_{e}$,
    \begin{equation}
        V_{M,\gamma}(\pi) \leq V_{M,\gamma_{e}}(\pi) \leq  V_{M,\gamma}(\pi) + \frac{\gamma_{e}-\gamma}{(1-\gamma)(1-\gamma_{e})}r_{\text{\rm max}},
    \end{equation}
    where $\gamma_{e}$ is the evaluation discount factor.
\end{lemma}
% \begin{proof}
%     See Appendix.
% \end{proof}
The bound above is tight in a trivial case, while it is usually very loose in practice.
Together, we have the following bound with a guidance discount factor $\gamma$ different from the true evaluation discount factor $\gamma_e$.
\begin{theorem}
    \label{theorem:1}
    %Suppose there exists an absolute constant %$c^\dagger >0$ such that with probability %$1-\xi/2$,
    %\begin{align}
    %    &\frac{1}{N} \cdot\sum_{\tau=1}^N{\phi(s_\tau,a_\tau)\phi(s_\tau,a_\tau)^\top}\succeq  \nonumber \\
    %    &c^\dagger \cdot  \EE_{\pi^*}\bigl[\phi(s_t,a_t)\phi(s_t,a_t)^\top\biggiven s_0=s\bigr], 
    %\end{align}

    %for all $s\in \cS$. In Algorithm~\ref{alg:1}, we set 
    %\begin{equation}
    %    \lambda =1, \quad \beta= c\cdot d V_{\text{\rm max}}\sqrt{\zeta}, \quad \zeta = \log{(4dN/(1-\gamma)\xi)},
    %\end{equation}
    Based on the same assumption and definition as in Lemma~\ref{lemma:2}, we set $\zeta=\log{(4dN/(1-\gamma)\xi)}$, $\beta=c \cdot d r_{\text{\rm max}}\sqrt{\zeta}/(1-\gamma)$ and $\lambda =1$.
    %where $V_{\text{\rm max}}=r_{\text{\rm max}}/(1-\gamma)$, $c>0$ is an absolute constant and $\xi \in (0,1)$ is the confidence parameter. 
    Then with probability $1-\xi$, the suboptimality bound of the policy $\widehat{\pi}$ generated by Algorithm~\ref{alg:1} satisfies
    \begin{align*}
     \text{\rm SubOpt}\big(\widehat{\pi};\gamma_e \big) 
    \leq &\frac{2c}{(1-\gamma)^2} \sqrt{c^\dagger d^3\zeta/N}\cdot r_{\text{\rm max}} \nonumber\\
    &+ \frac{\gamma_{e}-\gamma}{(1-\gamma)(1-\gamma_{e})}\cdot r_{\text{\rm max}}.
    \end{align*}
\end{theorem}
\begin{proof}
    The result follows immediately from Lemma~\ref{lemma:2} and Lemma~\ref{lemma:1}.
\end{proof}

Theorem~\ref{theorem:1} gives an upper bound for pessimistic offline algorithms with two terms. Both terms monotonically depend on the guidance discount factor $\gamma$ but in an opposite way, which suggests {\em there exists an optimal trade-off $\gamma^*\in [0, \gamma_{e}]$}.
It also suggests that this optimal trade-off $\gamma^*$ is dependent on other factors like the coverage ratio of the dataset and the size of the dataset. A small or poorly covered dataset (i.e., a large coverage coefficient) makes the first term's coefficient larger, requiring a lower discount factor to achieve optimal performance. We empirically observe this effect on both toy examples as well as large D4RL tasks, as shown in Section~\ref{experiments}.

\subsection{Pessimistic Effect}
This section analyses the pessimism effect of a lower discount factor. We show that, perhaps surprisingly, learning with a lower discount factor is equivalent to one type of the model-based pessimism mechanism, as depicted in Algorithm~\ref{alg:2}. This is characterized by the following lemma.
% \begin{lemma}
%     \label{lemma:3}
%     The optimal value function with a smaller discount factor is bounded by the model-based pessimistic value function. Formally, let
%     \begin{equation}
%         \label{model_based_policy_opt}
%         V_{\text{mb}}(\gamma,\varepsilon) = V_\gamma(\pi^*_{M_\varepsilon}), 
%     \end{equation}
%     where $\pi^*_{M_\varepsilon} \in \argmax_{\pi\in\Pi} \argmin_{M\in\mathcal{M}_\varepsilon} V_{M,\gamma}(\pi)$, and 
%     \begin{equation}
%         \label{small_gamma_policy_opt}
%         \mathcal{M}_\varepsilon = \set{M|D_{TV}(\cP_M(\cdot|s,a),\cP_{M_0}(\cdot|s,a))\leq \varepsilon, \forall s,a }, \notag
%     \end{equation}
%     then we have
%     \begin{equation}
%         V_{\text{mb}}(\gamma,2\varepsilon) \leq V^*_{M_0,(1-\varepsilon)\gamma}\leq V_{\text{mb}}(\gamma,2(1-p)\varepsilon),
%     \end{equation}
%     where $p=\sup_{s,a}\sum_{s'\in\cS_{\text{min},(1-\varepsilon)\gamma}}\cP(s'|s,a)$ and $\cS_{\text{min},\gamma}=\{s\in\cS\given V_{\text{min}}(s)=\min_s V^*_\gamma(s)\}$.
% \end{lemma}
\begin{lemma}
    \label{lemma:3}
    %The optimal value function with a smaller discount factor is equivalent to a special class of model-based pessimistic value function up to a constant.
    The optimal value function with a lower discount factor is equivalent to the pessimistic value function over a set of models.
    Formally, let
    \begin{equation}
    \label{model_based_policy_opt}
        \pi^*_{\mathcal{M}_\varepsilon} \in \argmax_{\pi} \min_{M\in\mathcal{M}_\varepsilon} V_{M,\gamma}(\pi),
    \end{equation}
    where
    \begin{equation}
        \label{small_gamma_policy_opt}
        \mathcal{M}_\varepsilon = \set{M| \cP_M(\cdot|s,a)= (1-\varepsilon)\cP_{M_0}(\cdot|s,a)+\varepsilon \cP(\cdot) }, \notag
    \end{equation}
    and $\cP(\cdot)$ is an arbitrary distribution over $\cS$, then we have
    \begin{equation}
        V^*_{M_0,(1-\varepsilon)\gamma}= V_{M_0,\gamma}(\pi^*_{\cM_\epsilon})+\Delta,
    \end{equation}
    where $\Delta$ is an absolute constant.
\end{lemma}

\begin{proof}
    See Appendix~\ref{proof_lemma_3} for a detailed proof.
\end{proof}

The equality in Lemma~\ref{lemma:3} shows that learning with a lower discount factor itself acts as a kind of model-based pessimism, which allows us to derive a bound without any other additional regularizations. We consider the model-based pessimism, where the model parameters are learned through maximum likelihood estimation (MLE). With the techniques in~\citep{geer2000empirical} that allow us to estimate the concentration rate of the MLE estimator, we have the following theorem. The proof of the following theorem is analogous to the analysis in~\citep{uehara2021pessimistic}.
\begin{theorem}
    \label{theorem:2}
    (\textit{informal}) Suppose there exists an absolute constant 
    \begin{align}
        \label{eq:event_opt_explore_2}
        c^\ddagger=\sup_{x\in\mathbb{R}^d} \frac{x^{\top}  \Sigma_{\pi^*} x}{x^{\top} \Sigma_\rho x } < \infty,
    \end{align} 
    $\Sigma_{\rho}=\EE_{\rho}[\phi(s,a)\phi(s,a)^{\top}],~\Sigma_{\pi^{*}}=\EE_{d^{\pi^{*}} }[\phi(s,a)\phi(s,a)^{\top}].$


    And suppose the underlying MDP follows the regularity condition in Assumption~\ref{assumption_regularity}. Set 
    $$\gamma = (1-\varepsilon)\gamma_e,~\varepsilon=c_1 \sqrt{d\zeta/N},\zeta = \log^2{(c_2Nd/\xi)}.$$
    Then, with probability $1-\xi$, Learning with a guidance discount factor $\gamma$ yields a policy $\hat{\pi}$ such that
    \begin{align}
        \text{\rm SubOpt}\big(\widehat{\pi};\gamma_e \big) \leq 
        \frac{c_3}{(1-\gamma_e)^{2}}\sqrt{c^\ddagger d^2 \zeta / N} \cdot r_{\text{max}},
    \end{align}
    % where $c^\ddagger=\sup_{x\in\mathbb{R}^d} \frac{x^{\top} \Sigma_\rho x}{x^{\top} \Sigma_{\pi^*} x }$, $\Sigma_{\rho}=\EE_{\rho}[\phi(s,a)\phi(s,a)^{\top}]$, $\Sigma_{\pi^{*}}=\EE_{d^{\pi^{*}} }[\phi(s,a)\phi(s,a)^{\top}]$, and $c_1,c_2,c_3$ are universal constants.
    where $c_1,c_2,c_3$ are constants.
\end{theorem}
\begin{proof}
    See Appendix~\ref{proof_theorem_2} for a detailed description and proof.
\end{proof}

Similar to $c^{\dagger}$ in Equation~\eqref{eq:event_opt_explore}, $c^{\ddagger}$ can be interpreted as another coverage coefficient, and the difference between $c^{\dagger}$ and $c^{\ddagger}$ are  technical. Theorem~\ref{theorem:2} shows that, with a properly chosen $\gamma$, we have a performance guarantee without any other offline techniques. We name this effect of the discount factor the pessimistic effect. 
Note that to make this bound meaningful, we need the dataset size $N$ to be large enough so that $1-\varepsilon >0$. This means that this theorem applies when the data is sufficient, contrary to the condition for the regularization effect. Compared to the bound in Theorem~\ref{theorem:1}, we note that the bound in Theorem~\ref{theorem:2} is smaller with a factor of $\sqrt{d}$ because a lower $\gamma$ resembles the model-based pessimism rather than a model-free one. 

We empirically verify this effect on the tabular MDPs and the D4RL dataset, where simple discount factor regularization is enough to derive a reasonable performance. 
% While the pessimism of lower $\gamma$ is not as good as the state-of-the-art offline algorithms, it serves as a good baseline. It significantly surpasses online algorithms with no discount factor pessimism. 
This pessimistic effect suggests that $\gamma$ affects the performance in offline RL differently compared to online settings.
